Act3D: 3D Feature Field Transformers for Multi-Task Robotic Manipulation

3D perceptual representations are well suited for robot manipulation as they easily encode occlusions and simplify spatial reasoning. Many manipulation tasks require high spatial precision in end-effector pose prediction, which typically demands high-resolution 3D feature grids that are computationally expensive to process. As a result, most manipulation policies operate directly in 2D, foregoing 3D inductive biases. In this paper, we introduce Act3D, a manipulation policy transformer that represents the robot's workspace using a 3D feature field with adaptive resolutions dependent on the task at hand. The model lifts 2D pre-trained features to 3D using sensed depth, and attends to them to compute features for sampled 3D points. It samples 3D point grids in a coarse to fine manner, featurizes them using relative-position attention, and selects where to focus the next round of point sampling. In this way, it efficiently computes 3D action maps of high spatial resolution. Act3D sets a new state-of-the-art in RL-Bench, an established manipulation benchmark, where it achieves 10% absolute improvement over the previous SOTA 2D multi-view policy on 74 RLBench tasks and 22% absolute improvement with 3x less compute over the previous SOTA 3D policy. We quantify the importance of relative spatial attention, large-scale vision-language pre-trained 2D backbones, and weight tying across coarse-to-fine attentions in ablative experiments. Code and videos are available on our project website: https://act3d.github.io/.

==> comments.tex <==
lets remove teaser figure
Lets expand task figure, else is not impressive, 3-4 rows would be great

==> old_related.tex <==
\section{Related Work}

% Short broader context
\subsection{Learning robot manipulation from demonstrations}
While early methods for robot manipulation such as visual servoing~\cite{hill1979real, chaumette2006visual} were designed manually, the need to cope with large variations in objects, scenes, environments, and goals led to the emergence of learning-based neural policies  \cite{levine2016end, finn2017deep, kalashnikov2018qt, jang2022bc}, recently leveraging Transformer architectures~\cite{shridhar2023perceiver, guhur2023instruction, liu2022instruction, brohan2022rt, shafiullah2022behavior} that learn to predict robot actions from video input and language instruction using reinforcement learning \cite{}, imitation learning \cite{} or a combination of the two \cite{}. 
%Two paradigms emerged to train manipulation policies: reinforcement learning (RL)~\cite{}, and learning from demonstrations~\cite{}; 
\model{} is trained with imitation learning. 
Out of the several simulation environments available for benchmarking \cite{}, we chose RLBench~\cite{james2020rlbench} for its diversity of 6 DoF manipulation tasks and ease of generating demonstrations with templated language goals.

% Focused related work that follows the flow of the intro with more details
% - End-to-end image-to-action
% - Transporter networks
% - Harder with 6 DoF actions: 3D voxelization (PerAct), predict offset (HiveFormer, etc)
% - Model to resolve this issue
% - Contrast with C2F-ARM, most closely related work 
\paragraph{Action detection inductive bias in manipulation policies}
%Solutions to many robotic manipulation tasks can be represented as a sequence of 6 DoF robot end-effector poses.


End-to-end image-to-action policy models, such as RT-1~\cite{brohan2022rt}, GATO~\cite{reed2022generalist}, BC-Z~\cite{jang2022bc}, and  InstructRL~\cite{liu2022instruction}, directly predict 6 DoF end-effector poses from 2D video input and language instructions, foregoing any 3D inductive biases. 
They are generally sample inefficient, requiring many thousands of demonstrations to learn spatial reasoning and generalize to new objects and environments, and remain brittle to camera viewpoint changes even at this scale.
Transporter networks \cite{} and their subsequent variants \cite{} formulate 4-DoF keypose prediction as pixel classification in 2D overhead images for tabletop scene rearrangement. 
This \emph{action detection} inductive bias that predicts robot actions by classification of local features instead of regression, makes these models  more sample efficient. 
However, they are limited to top-down 2D planar worlds with simple pick-and-place primitives. 
Implementing action detection fully in 3D is more challenging than in 2D overhead images because end-effector 3D poses often need to be predicted on 3D points in the empty space, not just in contact with the 3D physical scene points. 
This requires featurizing points in the empty 3D space.
3D policy models of C2F-ARM~\cite{james2022coarse} and PerAct~\cite{shridhar2023perceiver} voxelize the robot workspace and are trained to detect the 3D voxel that contains the next end-effector keypose. 
However, 3D voxelization suffers from a high computational cost caused by increasing the 3D resolution of the voxel grid, which is necessary for spatially precise 3D pose prediction. 
Coarse-to-fine voxelization, as in C2F-ARM, partially addresses this issue but [...]
\topic{Theo: What's our story for why coarse-to-fine voxelization of C2F-ARM is worse than our approach? In our method, fine ghost point sampling stages don't attend to coarse global visual tokens but to local fine visual tokens, just like C2F-ARM}
HiveFormer~\cite{guhur2023instruction}, Auto-$\lambda$~\cite{liu2022auto} and SLAP~\cite{parashar2023spatial} work around this issue by avoiding featurizing points in the empty space and instead detecting a contact point in the physical 3D feature cloud and then regressing an offset from this contact point towards the end-effector predicted position. 
This is a reasonable design choice but it does not fully exploit the action detection inductive bias. 
\model{} avoids voxelization altogether, and proposes a coarse-to-fine sampling of the empty 3D space, where increasingly finer 3D point grids are sampled and featurized with relative attention to the 3D physical scene feature cloud. In this way, infinite 3D spatial resolution can be achieved during end-effector 3D position prediction. 
\model{} outperforms PerAct by a large margin while requiring 3x less compute to train.


% Should we include this to stress the fact that we can easily leverage pre-trained 2D backbones? PerAct related works is good about this
%\paragraph{Object-centric representations in manipulation policies}
%- Traditional pipeline: compounding errors
%- More flexible object-centric representations help with some tasks (VIMA, MOO) but not general enough for all tasks (defornmables, beans, etc)
%- Features from pre-trained 2D backbones can help with visual and language generalization without imposing object structure
%- Model doesn't use any object-centric representations for generality, easily extensible with object visual tokens in physical scene feature cloud in future work





















\section{Related Work}

\paragraph{Learning robot manipulation from demonstrations}


For
benchmarking, several simulation environments exist [70, 17, 53], but we use RLBench [15] for its
diversity of 6-DoF tasks and ease of generating demonstrations with templated language goals.


While other
works in 6-DoF grasping [32, 33, 34, 35, 36, 37] have used RGB-D and pointcloud input, they
have not been applied to sequential tasks or used with language-conditioning. 

Another line of work
tackles data inefficiency by using pre-trained image representations [16, 38, 39] to bootstrap BC.
Although our framework is trained from scratch, such pre-training approaches could be integrated
together in future works for even greater efficiency and generalization to unseen objects.




\paragraph{Inductive biases in manipulation policies}
\todo{THEO-Xian}
\todo{THEO-Xian}
Solutions to many robotic manipulation tasks can be represented as a sequence of 6 DoF robot end-effector   poses. Many recent methods train manipulation policies to predict such end-effector 3D poses from sensory input and a language instruction 
%using supervision from demonstration trajectories
~\cite{shridhar2023perceiver, guhur2023instruction, liu2022instruction, james2022coarse, brohan2022rt}, using imitation or reinforcement learning. 

%https://arxiv.org/pdf/2209.05451.pdf

%and Transformers~\cite{vaswani2017attention} have shown promise in predicting these poses from 
%videos and language instructions
%sensory input~\cite{shridhar2023perceiver, guhur2023instruction, liu2022instruction, james2022coarse, brohan2022rt}. 


%However, Transformer architectures for manipulation policies vary in their use of space.
%are often formulated as an image-to-action prediction task. Training directly on RGB
%images for 6-DoF tasks is often inefficient, 



End-to-end image-to-action policy models, such as RT-1~\cite{brohan2022rt}, GATO~\cite{reed2022generalist}, BC-Z~\cite{jang2022bc}, and  InstructRL~\cite{liu2022instruction}, \todo{Hiveformer??} directly predict 6 DoF end-effector poses from 2D video input and language instructions, foregoing any 3D or other inductive biases.  They are generally sample inefficient, require often thousands of several demonstrations, and cannot easily generalize across camera viewpoints.

 Transporter networks \cite{} and their subsequent variants \cite{} formulate robot keypose prediction as pixel classification in re-projected from BEV images, for table top scene re-arrangement. This  \emph{action detection} inductive bias that predicts robot actions by classification of local features instead of regression, has shown to make these models much more sample efficient. However, these models are limited to top-down 2D planar worlds with simple pick-and-place primitives. 

 %\emph{action detection} inductive bias~\cite{florence2022implicit} based on which visual features relevant for robot pose detection are locally associated to the \todo{what does this citation say about that bias?} and are more robust to camera view changes.
%The question arises: can we combine the best of both worlds? 
%In other words, how can we extend the action detection inductive bias of Transporter Networks~\cite{zeng2021transporter} to broader 6 DoF manipulation while leveraging pre-trained 2D backbones and preserving computational efficiency?

 
 %However, they can only handle pick n place tasks in 2D planar worlds. 
 
 %Similar action detection inductive bias had been earlier  proposed by transporter networks and its variants \cite{} for robot rearrangement of 2D planar worlds from a bird's eye view reporjected image. 
 
 %to learn basic skills like rearranging objects. 

%They typically leverage pre-trained vision-and-language backbones \cite{}. 

 
 3D policy models of PerAct~\cite{shridhar2023perceiver}, C2F-ARM~\cite{james2022coarse}, or SLAP~\cite{parashar2023spatial}, 
have attempted to generalise action detection to general 3D tasks.  
 They geometrically fuse 2.5 point clouds  from depth sensors from one or multiple viewpoints into a 3D scene point cloud,  
 %2D image information into 3D feature grids using depth and camera instrinsics and extrinsics, 
 and %predict  3D end-effector keyposes using  3D  neural operations over a voxelized 3D space. They 
 are trained to predict the 3D voxel that contains the next end-effector keypose. They typically enjoy  better sample efficiency and are 
 %thanks to the action detection and 3D inductive bias that fuses information using parameter free geometric operations across views, which also helps them to be 
 robust to camera view changes thanks to geometric aggregation of per view information.  
However,
%3D grids or point clouds can be very expensive to process and manipulation often requires highly accurate robot end-effector localization.
 3D voxelization suffers from the intractability caused by increasing the 3d resolution of the voxel grid, which is necessary for highly accurate 3d pose prediction. C2F-ARM proposes a coarse-to-fine voxelization scheme, which a limited receptive field and  does not attend to the full 3D voxel grid during finer grid iterations. Per-act using perceiver's global attention operation, which in place of all voxel-to-voxel attention, which grows quadratically to the number of voxels, use voxel-to-set latent attention, where  voxel tokens attends to a constant number of learnt latent vectors, and voxel to voxel information propagation happens through the selt latent self attentions and set latent to voxel attentions. 
 
 \model{} avoids voxelization altogether, and proposes a coarse-to-fine sampling of the empty 3D space, where at each iteration a 3D point grid is sampled, and the sampled 3D points attend to all 3D point tokens. In this way, infinite 3D spatial resolution can be achieved during end-effector 3D location prediction. It outperforms Per-act by a large margin while being 10X faster. It thus is a general vision-language manipulation 3D transformer for scalable learning from demonstrations. % much faster and much more




 %The coarse-to-fine-grain scheme has a limited receptive field that cannot look at the entire scene at the finest level.
 %within the action condition 
 %with the late%and attention is carried out across these co
 
 % use the action detection 
 
 
 %\todo{is that correct?}
 %\emph{detect actions} in the workspace, inspired by the successes of Transporter Networks~\cite{zeng2021transporter} and CLIPort~\cite{shridhar2022cliport} for tabletop manipulation from top-down views. 
%The former set of methods typically leverage pre-trained vision-and-language backbones and are efficient in compute and memory, 
%while the latter set of methods 

%, that voxelization 
%, and 

%locality of computation



%Guiding multi-step rearrangement tasks with natural language instructions.


%Vision for Manipulation. 

%
%In 3D, James et al. proposed C2FARM [14], an
%action-centric reinforcement learning (RL) agent with a coarse-to-


% In contrast, PERACT uses a voxelized observation
%and action space, which is dramatically more efficient and robust in 6-DoF settings. 






%Transformers for Agents and Robots. Transformers have become the prevalent architecture in several domains. Starting with NLP [2, 3, 40], recently in vision [4, 41], and even RL [8, 42, 43]. In robotics, Transformers have been applied to assistive teleop [44], legged locomotion [45], pathplanning [46, 47], imitation learning [48, 49], morphology controllers [50], spatial rearrangement [51], and grasping [52]. 


%Transformers have also achieved impressive results in multi-domain settings like in Gato [9] where a single Transformer was trained on 16 domains such as captioning, language-grounding, robotic control etc. 

%However, Gato relies on extremely large datasets like 15K episodes for block stacking and 94K episodes for Meta-World [53] tasks. Our approach might complement agents like Gato, which could use our 3D formulation for greater efficiency and robustness.


%Language Grounding for Manipulation. Several works have proposed methods for grounding language in robot actions [54, 55, 56, 57, 58, 59, 60, 61, 62, 63, 64, 65]. However, these methods use disentangled pipelines for perception and action, with the language primarily being used to guide perception [66]. Recently, a number of end-to-end approaches [13, 12, 67, 68, 69] have been proposed for conditioning BC agents with language instructions. These methods require thousands of human demos or autonomous episodes that are collected over several days or even months. In contrast, PERACT can learn robust multi-task policies with just a few minutes of training data. 



